Graph Resistance and Learning from Pairwise Comparisons

We consider the problem of learning the qualities of a collection of items by performing noisy comparisons among them. Following the standard paradigm, we assume there is a fixed "comparison graph" and every neighboring pair of items in this graph is compared $k$ times according to the Bradley-Terry-Luce model (where the probability than an item wins a comparison is proportional the item quality). We are interested in how the relative error in quality estimation scales with the comparison graph in the regime where $k$ is large. We prove that, after a known transition period, the relevant graph-theoretic quantity is the square root of the resistance of the comparison graph. Specifically, we provide an algorithm that is minimax optimal. The algorithm has a relative error decay that scales with the square root of the graph resistance, and provide a matching lower bound (up to log factors). The performance guarantee of our algorithm, both in terms of the graph and the skewness of the item quality distribution, outperforms earlier results.

==> declarations.tex <==
\bibliographystyle{plain}


%%%%%%%%% various packages %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{hyperref}
\usepackage{amssymb,amsmath}
\usepackage{amsfonts}
\usepackage[english]{babel}
\usepackage[utf8]{inputenc}
\usepackage{fancyhdr}
\usepackage{yfonts}
\usepackage{mathrsfs}
\usepackage[dvips]{graphicx}
\usepackage{enumerate}
\usepackage{xspace}
%\usepackage[rflt]{floatflt}
\usepackage{cite}
%\usepackage{amsthm}

%\usepackage{algorithm}
%\floatname{algorithm}{Alg.}
%\usepackage{algorithmic}
\usepackage{psfrag}
\usepackage{url}


%%%%%%%%% Commenting commands %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\providecommand{\margincom}[1]{\marginpar{{\small#1}}}

\usepackage[dvipsnames]{xcolor}

%\newcommand{\sam}[1]{\YellowOrange{#1}}
%\newcommand{\sam}[1]{\blue{#1}}
\newcommand{\sam}[1]{{\leavevmode\color{blue}{#1}}}
\providecommand{\comsam[1]}{\sam{\com{SAM}{#1}}}
\newcommand{\jh}[1]{{#1}}
%\newcommand{\jh}[1]{\blue{#1}}
\providecommand{\comjh[1]}{\jh{\textcolor{blue}{\com{JH}{#1}}}}
\providecommand{\com[2]}{\begin{tt}[#1: #2]\end{tt}}
\usepackage{color}
\newcommand{\JMH}[1]{#1}
\newcommand{\modif}[1]{{#1}}
%\newcommand{\modif}[1]{{\color{red} #1}}
\newcommand{\jnt}[1]{{#1}}
%\newcommand{\del}[1]{{DELETE:\color{yellow} #1}}

%%%%%%%%%%%% "Theorems" %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newtheorem{prop}{Proposition}%[section]
%\newtheorem{thm}{Theorem}%[section]
%\newtheorem{defi}{Definition}%[section]
%\newtheorem{cor}{Corollary}%[section]
%\newtheorem{conj}{Conjecture}%[section]
%\newtheorem{lem}{Lemma}%[section]
%\newtheorem{ass}{Assumption}%[section]
%\newtheorem{ex}{Example}%[section]
%\newtheorem{prob}{Problem}%[section]
%\newtheorem{question}{Question}%[section]
%\newtheorem{rem}{Remark}%[section]




\providecommand{\sol[1]}{\vspace{.5cm}\noindent {\textbf{Solution de l'exercice #1}}\\}


%%%%%%%%%%%%% Mathematical macros %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\providecommand{\prt}[1]{\left( #1 \right)}
\providecommand{\C}{\mathbb{C}} 
\providecommand{\PP}{\mathbb{P}}
\providecommand{\e}{\phantom{aaa}}
\providecommand{\abs[1]}{\left|#1\right|}
\providecommand{\norm[1]}{\abs{\abs{#1}}}%
\providecommand{\floor[1]}{\lfloor  #1 \rfloor }
\providecommand{\ceil[1]}{\lceil #1  \rceil}
\providecommand{\1}{\textbf{1}}
\providecommand{\0}{\textbf{0}}\providecommand{\quotes[1]}{``#1"}
\providecommand{\scalprod[2]}{\left<#1,#2\right>}%
\providecommand{\Linf}{{\mathcal{L}_\infty}}
\providecommand{\sign}[1]{\mathrm{sign}\prt{#1}}

\providecommand{\L}{{\mathcal{L}}}
%\mathbf{sign}\mathit{sign}sign \mathtt{sign}\mathsf{sign}\mathrm{sign}



\providecommand{\matr[4]}{\left(\begin{array}{cc}#1 & #2 \\ #3
&#4\end{array}\right) }
\providecommand{\hvec[2]}{\left(\begin{array}{cc}#1 &
#2\end{array}\right) }
\providecommand{\vvec[2]}{\left(\begin{array}{c}#1 \\
#2\end{array}\right) }




\def\0{{\bf 0}}
\def\R{\mathbb{R}}
\def\N{\mathbb{N}}
\def\Z{\mathbb{Z}}
\def\Q{\mathbb{Q}}
\def\I{{\bf I}}
 \def\V{\mathcal{V}}
 \def\M{\mathcal{M}}
  \def\S{\mathcal{S}}
 \def\U{\mathcal{U}}
 \def\C{\mathcal{C}}
\def\G{\mathcal{G}}
\def\T{\mathcal{T}}
\def\EE{\mathcal{E}}
\def\E{\mathbb{E}}
\def\DD{\mathcal{D}}
\def\NN{\mathcal{N}}
%\def\T{\mathcal{T}}   %reset+switch set
%\def\J{\mathcal{J}}
%\def\E{\mathcal{E}}
%\def\S{\mathcal{S}}
%\def\II{\mathcal{I}}
%\def\O{\mathcal{O}}
%\def\F{\mathcal{F}}
%\def\e{\mbox{e}}
\newcommand{\unn}{\{1,\ldots, n\}}
\newcommand{\ie}{{\it i.e. }}
\newcommand\TODO[1]{\textbf{TODO: \textit{#1}}}

\newcommand{\ssum}{\displaystyle\sum}
\newcommand{\Var}[1]{\text{Var}{#1}}

%\usepackage{stackengine}
%\newcommand\simstack[1]{\mathrel{\stackunder[2pt]{\sim}{$\scriptscriptstyle#1$}}}

%\newcommand{\rpm}{\sbox0{$1$}\sbox2{$\pm$}
%  \raise\dimexpr(\ht0-\ht2)/2\relax\box2 }
\newcommand{\rpm}{\raisebox{.2ex}{$\scriptstyle\pm$}}
\newcommand{\ooneovern}{o\left(\frac{1}{n}\right)}
